Learning Latent and Hierarchical Structures in Cognitive Diagnosis Models

Cognitive Diagnosis Models (CDMs) are a special family of discrete latent variable models that are widely used in modern educational, psychological, social and biological sciences. A key component of CDMs is a binary $Q$-matrix characterizing the dependence structure between the items and the latent attributes. Additionally, researchers also assume in many applications certain hierarchical structures among the latent attributes to characterize their dependence. In most CDM applications, the attribute-attribute hierarchical structures, the item-attribute $Q$-matrix, the item-level diagnostic model, as well as the number of latent attributes, need to be fully or partially pre-specified, which however may be subjective and misspecified as noted by many recent studies. This paper considers the problem of jointly learning these latent and hierarchical structures in CDMs from observed data with minimal model assumptions. Specifically, a penalized likelihood approach is proposed to select the number of attributes and estimate the latent and hierarchical structures simultaneously. An efficient expectation-maximization (EM) algorithm and a latent structure recovery algorithm are developed, and statistical consistency theory is also established under mild conditions. The good performance of the proposed method is illustrated by simulation studies and a real data application in educational assessment.

==> manuscript.wordcount.tex <==
File: manuscript.tex
Encoding: utf8
Sum count: 11048
Words in text: 9924
Words in headers: 57
Words outside text (captions, etc.): 381
Number of headers: 18
Number of floats/tables/figures: 15
Number of math inlines: 660
Number of math displayed: 26
Subcounts:
  text+headers+captions (#headers/#floats/#inlines/#displayed)
  192+10+0 (2/0/2/0) _top_
  1045+1+0 (1/0/8/0) Section: Introduction
  53+2+0 (1/0/4/0) Section: Model Setup
  911+4+35 (1/2/88/5) Subsection: Hierarchical Cognitive Diagnosis Models
  286+6+0 (1/0/22/1) Subsection: CDMs as Restricted Latent Class Models
  0+3+0 (1/0/0/0) Section: Regularized Estimation Method
  1464+4+49 (1/2/85/7) Subsection: Motivation and Proposed Method
  1184+2+5 (1/1/158/3) Subsection: Theoretical Proporties
  0+2+0 (1/0/0/0) Section: Learning Algorithms
  494+3+9 (1/0/52/7) Subsection: Penalized EM Algorithm
  1054+5+53 (1/4/99/3) Subsection: Recover Latent Hierarchies and $Q$-matrix
  1397+2+121 (1/3/86/0) Section: Simulation Studies
  0+3+0 (1/0/0/0) Section: Real Data Analysis
  800+4+92 (1/2/33/0) Subsection: Analysis of ECPE Data
  461+4+17 (1/1/20/0) Subsection: Analysis of PISA Data
  545+1+0 (1/0/3/0) Section: Discussion
  38+1+0 (1/0/0/0) Section: Acknowledgments


